Digging Into Self-Supervised Monocular Depth Estimation

Per-pixel ground-truth depth data is challenging to acquire at scale. To overcome this limitation, self-supervised learning has emerged as a promising alternative for training models to perform monocular depth estimation. In this paper, we propose a set of improvements, which together result in both quantitatively and qualitatively improved depth maps compared to competing self-supervised methods. Research on self-supervised monocular training usually explores increasingly complex architectures, loss functions, and image formation models, all of which have recently helped to close the gap with fully-supervised methods. We show that a surprisingly simple model, and associated design choices, lead to superior predictions. In particular, we propose (i) a minimum reprojection loss, designed to robustly handle occlusions, (ii) a full-resolution multi-scale sampling method that reduces visual artifacts, and (iii) an auto-masking loss to ignore training pixels that violate camera motion assumptions. We demonstrate the effectiveness of each component in isolation, and show high quality, state-of-the-art results on the KITTI benchmark.

==> figs/texture_copy/texture_copy.tex <==
\newcommand{\turnwidth}{0.49\columnwidth}
\centering

\renewcommand{\arraystretch}{0}
\setlength\tabcolsep{0pt}


\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\begin{tabular}{C{0.5\columnwidth}c}

\small{Input} & \small{\textbf{Ours} (full) M} \\
\multicolumn{2}{c}{\includegraphics[width=1.0\columnwidth]{figs/texture_copy/texture_copy_fig.pdf}} \\


\small{Ours w/o min.~reprojection} & \small{Ours w/o full-res multi-scale}

\end{tabular}


==> supp_figs/motion/motion_figure.tex <==
\newcommand{\turnheightnew}{0.195\columnwidth}

\centering

\begin{tabular}{@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{}}

{\rotatebox{90}{\hspace{7mm}Input}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_color.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_color.jpg}\\

{\rotatebox{90}{\hspace{2mm}Zhou \ea~\cite{zhou2017unsupervised}}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_zhou_disp.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_zhou_disp.jpg} \\

{\rotatebox{90}{\hspace{4mm}DDVO~\cite{wang2017learning}}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_posenet_ddvo_disp.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_posenet_ddvo_disp.jpg} \\

{\rotatebox{90}{\hspace{0mm}\tiny{Mahjourian \ea~\cite{mahjourian2018unsupervised}}}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_google_icp_disp.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_google_icp_disp.jpg} \\

{\rotatebox{90}{\hspace{4mm}GeoNet~\cite{geonet2018}}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_geonet_disp.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_geonet_disp.jpg} \\

{\rotatebox{90}{\hspace{5mm}\textbf{Ours M}}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_ours_disp.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_ours_disp.jpg} \\

{\rotatebox{90}{\hspace{0mm}\textbf{Ours C+K M}}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_ours_city2kitti_disp.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_ours_city2kitti_disp.jpg} \\

{\rotatebox{90}{\hspace{4mm}\textbf{Ours MS}}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_ours_mixed_disp.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_ours_mixed_disp.jpg} \\

{\rotatebox{90}{\hspace{0mm}\textbf{Ours C+K MS}}} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/444_ours_city2kitti_mixed_disp.jpg} &
\includegraphics[height=\turnheightnew]{supp_figs/motion/689_ours_city2kitti_mixed_disp.jpg} \\

\end{tabular}

